Distributed Enforcement of Service Choreographies

Modern service-oriented systems are often built by reusing, and composing together, existing services distributed over the Internet. Service choreography is a possible form of service composition whose goal is to specify the interactions among participant services from a global perspective. In this paper, we formalize a method for the distributed and automated enforcement of service choreographies, and prove its correctness with respect to the realization of the specified choreography. The formalized method is implemented as part of a model-based tool chain released to support the development of choreography-based systems within the EU CHOReOS project. We illustrate our method at work on a distributed social proximity network scenario.

==> eptcsdata.tex <==
\providecommand{\firstpage}{18}
\providecommand{\publicationstatus}{Javier C\'amara and Jos\'e Proen\c{c}a (Eds.):\\
13th International Workshop on Foundations of\\
Coordination Languages and Self-Adaptive Systems (FOCLASA'14)\\
EPTCS 175, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.175.2}{10.4204/EPTCS.175.2}}
\pdfoutput=1

